Parton distribution functions and benchmark cross sections at NNLO

We present a determination of parton distribution functions (ABM11) and the strong coupling constant alpha_s at next-to-leading order and next-to-next-to-leading order (NNLO) in QCD based on world data for deep-inelastic scattering and fixed-target data for the Drell-Yan process. The analysis is performed in the fixed-flavor number scheme for n_f=3,4,5 and uses the MSbar-scheme for alpha_s and the heavy-quark masses. At NNLO we obtain the value alpha_s(M_Z) = 0.1134 +- 0.0011. The fit results are used to compute benchmark cross sections at hadron colliders to NNLO accuracy and to compare to data from the LHC.

==> ccfr <==
Parton distribution functions and benchmark cross sections at NNLO
S. Alekhin, J. Bluemlein and S. Moch

This file contains the data and systematic uncertainties (see Sec. 3 for details and use in PDF fit)
for the experiment
...
CCFR:  PR D64, 112006 (2001)

The data on the reduced DIS dimuon production cross sections 

sig=[(1-y-(xyM_N)^2/Q2) F_2 + y^2/2 F_T +- y(1-y/2) xF_3] B_mu

and the correction for unmeasured phase space \eta (not applied to the data)

The correlated systematic errors come from 1 source. All uncertainties are given in percent.

      x         Q2         y          sig     unc   \eta   NSE systematic uncertainty

neutrino beam

  0.230E-01  0.151E+01  0.320E+00  0.589E-01 21.90  0.464   1  3.06
  0.570E-01  0.375E+01  0.320E+00  0.619E-01 17.77  0.466   1  0.65
  0.100E+00  0.658E+01  0.320E+00  0.470E-01 17.45  0.470   1  0.85
  0.167E+00  0.110E+02  0.320E+00  0.495E-01 16.36  0.474   1  0.61
  0.336E+00  0.221E+02  0.320E+00  0.159E-01 15.09  0.491   1  0.63
  0.230E-01  0.270E+01  0.570E+00  0.137E+00 16.33  0.665   1  1.32
  0.570E-01  0.668E+01  0.570E+00  0.101E+00 15.76  0.667   1  0.79
  0.100E+00  0.117E+02  0.570E+00  0.706E-01 14.59  0.670   1  3.26
  0.167E+00  0.196E+02  0.570E+00  0.473E-01 14.16  0.675   1  2.11
  0.336E+00  0.394E+02  0.570E+00  0.226E-01 15.04  0.687   1  1.33
  0.230E-01  0.376E+01  0.795E+00  0.141E+00 15.85  0.752   1  3.13
  0.570E-01  0.932E+01  0.795E+00  0.136E+00 14.90  0.753   1  1.18
  0.100E+00  0.163E+02  0.795E+00  0.114E+00 15.06  0.756   1  1.23
  0.167E+00  0.273E+02  0.795E+00  0.812E-01 16.75  0.759   1  2.22
  0.336E+00  0.549E+02  0.795E+00  0.211E-01 18.96  0.768   1  1.42
  0.230E-01  0.290E+01  0.320E+00  0.133E+00 17.56  0.682   1  0.38
  0.570E-01  0.719E+01  0.320E+00  0.116E+00 16.55  0.683   1  3.10
  0.100E+00  0.126E+02  0.320E+00  0.931E-01 15.79  0.686   1  0.54
  0.167E+00  0.211E+02  0.320E+00  0.567E-01 15.87  0.690   1  0.53
  0.336E+00  0.424E+02  0.320E+00  0.254E-01 14.96  0.705   1  1.57
  0.230E-01  0.517E+01  0.570E+00  0.157E+00 15.72  0.810   1  0.45
  0.570E-01  0.128E+02  0.570E+00  0.167E+00 16.38  0.813   1  0.78
  0.100E+00  0.225E+02  0.570E+00  0.138E+00 16.36  0.815   1  0.51
  0.167E+00  0.375E+02  0.570E+00  0.912E-01 16.45  0.818   1  0.99
  0.336E+00  0.755E+02  0.570E+00  0.261E-01 16.48  0.826   1  0.77
  0.230E-01  0.721E+01  0.795E+00  0.164E+00 14.85  0.865   1  1.71
  0.570E-01  0.179E+02  0.795E+00  0.158E+00 15.23  0.866   1  0.63
  0.100E+00  0.313E+02  0.795E+00  0.109E+00 16.58  0.867   1  0.37
  0.167E+00  0.523E+02  0.795E+00  0.814E-01 16.46  0.869   1  0.37
  0.336E+00  0.105E+03  0.795E+00  0.230E-01 17.83  0.874   1  1.30
  0.230E-01  0.460E+01  0.320E+00  0.155E+00 15.14  0.785   1  0.32
  0.570E-01  0.114E+02  0.320E+00  0.161E+00 15.87  0.786   1  0.68
  0.100E+00  0.200E+02  0.320E+00  0.101E+00 15.59  0.789   1  1.69
  0.167E+00  0.334E+02  0.320E+00  0.619E-01 15.35  0.794   1  0.65
  0.336E+00  0.672E+02  0.320E+00  0.292E-01 14.04  0.804   1  1.03
  0.230E-01  0.819E+01  0.570E+00  0.181E+00 16.56  0.877   1  0.83
  0.570E-01  0.203E+02  0.570E+00  0.169E+00 17.68  0.878   1  0.35
  0.100E+00  0.356E+02  0.570E+00  0.154E+00 17.71  0.880   1  5.27
  0.167E+00  0.595E+02  0.570E+00  0.712E-01 17.70  0.882   1  0.56
  0.336E+00  0.120E+03  0.570E+00  0.285E-01 16.84  0.888   1  5.61
  0.230E-01  0.114E+02  0.795E+00  0.242E+00 14.13  0.915   1  0.99
  0.570E-01  0.283E+02  0.795E+00  0.205E+00 15.64  0.916   1  0.20
  0.100E+00  0.497E+02  0.795E+00  0.169E+00 16.88  0.916   1  0.30
  0.167E+00  0.829E+02  0.795E+00  0.948E-01 16.77  0.918   1  0.21
  0.336E+00  0.167E+03  0.795E+00  0.328E-01 18.29  0.921   1  0.61  

anti-neutrino beam

  0.400E-01  0.234E+01  0.356E+00  0.483E-01 37.68  0.417   1  5.59
  0.680E-01  0.398E+01  0.356E+00  0.484E-01 35.33  0.418   1  1.86
  0.109E+00  0.638E+01  0.356E+00  0.342E-01 35.38  0.421   1 43.86
  0.206E+00  0.120E+02  0.356E+00  0.140E-01 33.57  0.425   1  0.71
  0.170E-01  0.166E+01  0.596E+00  0.117E+00 33.30  0.612   1  5.29
  0.400E-01  0.392E+01  0.596E+00  0.115E+00 32.03  0.613   1  2.78
  0.680E-01  0.666E+01  0.596E+00  0.660E-01 31.21  0.614   1  3.18
  0.109E+00  0.107E+02  0.596E+00  0.684E-01 32.02  0.616   1  9.50
  0.206E+00  0.202E+02  0.596E+00  0.173E-01 32.37  0.622   1  2.31
  0.170E-01  0.224E+01  0.803E+00  0.117E+00 35.71  0.702   1 10.04
  0.400E-01  0.528E+01  0.803E+00  0.928E-01 33.73  0.703   1  7.87
  0.680E-01  0.897E+01  0.803E+00  0.974E-01 35.32  0.704   1  5.65
  0.109E+00  0.144E+02  0.803E+00  0.912E-01 34.10  0.707   1  3.62
  0.206E+00  0.272E+02  0.803E+00  0.305E-01 38.69  0.710   1  1.64
  0.170E-01  0.183E+01  0.356E+00  0.101E+00 39.21  0.637   1  3.07
  0.400E-01  0.430E+01  0.356E+00  0.119E+00 34.87  0.636   1  6.39
  0.680E-01  0.731E+01  0.356E+00  0.867E-01 35.06  0.639   1  3.46
  0.109E+00  0.117E+02  0.356E+00  0.609E-01 33.83  0.641   1  0.66
  0.206E+00  0.221E+02  0.356E+00  0.228E-01 32.46  0.645   1  5.70
  0.170E-01  0.306E+01  0.596E+00  0.159E+00 35.55  0.769   1  5.78
  0.400E-01  0.719E+01  0.596E+00  0.152E+00 34.78  0.770   1  5.59
  0.680E-01  0.122E+02  0.596E+00  0.114E+00 35.49  0.772   1  4.63
  0.109E+00  0.196E+02  0.596E+00  0.640E-01 35.47  0.774   1  1.09
  0.206E+00  0.370E+02  0.596E+00  0.219E-01 34.25  0.777   1  0.46
  0.170E-01  0.412E+01  0.803E+00  0.183E+00 31.58  0.828   1 10.18
  0.400E-01  0.969E+01  0.803E+00  0.173E+00 34.26  0.829   1  7.55
  0.680E-01  0.165E+02  0.803E+00  0.182E+00 33.21  0.829   1  3.52
  0.109E+00  0.264E+02  0.803E+00  0.789E-01 34.85  0.832   1  3.17
  0.206E+00  0.499E+02  0.803E+00  0.225E-01 36.44  0.833   1  1.78
  0.170E-01  0.302E+01  0.356E+00  0.229E+00 31.98  0.763   1  0.31
  0.400E-01  0.711E+01  0.356E+00  0.132E+00 34.14  0.762   1  1.06
  0.680E-01  0.121E+02  0.356E+00  0.138E+00 32.22  0.764   1  0.58
  0.109E+00  0.194E+02  0.356E+00  0.619E-01 32.47  0.765   1  0.81
  0.206E+00  0.366E+02  0.356E+00  0.161E-01 31.68  0.770   1  7.45
  0.170E-01  0.506E+01  0.596E+00  0.284E+00 35.79  0.854   1  3.59
  0.400E-01  0.119E+02  0.596E+00  0.185E+00 36.65  0.854   1  1.14
  0.680E-01  0.202E+02  0.596E+00  0.125E+00 38.35  0.856   1  0.88
  0.109E+00  0.324E+02  0.596E+00  0.101E+00 38.64  0.857   1  0.30
  0.206E+00  0.613E+02  0.596E+00  0.262E-01 37.02  0.860   1  0.38
  0.170E-01  0.681E+01  0.803E+00  0.254E+00 29.50  0.894   1  8.66
  0.400E-01  0.160E+02  0.803E+00  0.152E+00 34.21  0.895   1  3.96
  0.680E-01  0.273E+02  0.803E+00  0.792E-01 37.50  0.895   1  4.92
  0.109E+00  0.437E+02  0.803E+00  0.569E-01 36.03  0.897   1  3.34
  0.206E+00  0.826E+02  0.803E+00  0.275E-01 37.82  0.898   1  0.36 


==> fnal-e605 <==
Parton distribution functions and benchmark cross sections at NNLO
S. Alekhin, J. Bluemlein and S. Moch

This file contains the data and systematic uncertainties (see Sec. 3 for details and use in PDF fit)
for the experiment
...
FNAL-E605: PR D43, 2815 (1991)

The data on the DY process cross section

S*d2(sig)/d(sqrt(tau))/d(Y) [nb*GeV^2]

The correlated systematic errors come from 2 sources including the
normalization. All uncertainties are given in percent.

  sqrt(\tau)    Y          sig     unc   NSE systematic uncertainties

  0.183E+00 -0.200E+00  0.364E+03 29.12   2 15.00  9.79
  0.188E+00 -0.200E+00  0.209E+03 21.96   2 15.00  9.39
  0.194E+00 -0.200E+00  0.220E+03 18.32   2 15.00  8.98
  0.199E+00 -0.200E+00  0.243E+03 18.72   2 15.00  8.59
  0.204E+00 -0.200E+00  0.119E+03 18.07   2 15.00  8.19
  0.209E+00 -0.200E+00  0.176E+03 17.73   2 15.00  7.79
  0.214E+00 -0.200E+00  0.174E+03 16.38   2 15.00  7.39
  0.219E+00 -0.200E+00  0.140E+03 14.14   2 15.00  6.99
  0.224E+00 -0.200E+00  0.105E+03 12.76   2 15.00  6.59
  0.230E+00 -0.200E+00  0.123E+03 11.30   2 15.00  6.18
  0.271E+00 -0.200E+00  0.349E+02 12.38   2 15.00  2.99
  0.276E+00 -0.200E+00  0.289E+02 14.91   2 15.00  2.58
  0.281E+00 -0.200E+00  0.274E+02 15.80   2 15.00  2.18
  0.291E+00 -0.200E+00  0.162E+02 10.00   2 15.00  1.38
  0.312E+00 -0.200E+00  0.107E+02 10.28   2 15.00 -0.22
  0.343E+00 -0.200E+00  0.357E+01 15.85   2 15.00 -2.62
  0.384E+00 -0.200E+00  0.170E+01 27.47   2 15.00 -5.82
  0.183E+00 -0.100E+00  0.399E+03 21.33   2 15.00  9.79
  0.188E+00 -0.100E+00  0.315E+03 17.62   2 15.00  9.39
  0.194E+00 -0.100E+00  0.277E+03 16.39   2 15.00  8.98
  0.199E+00 -0.100E+00  0.244E+03 14.34   2 15.00  8.59
  0.204E+00 -0.100E+00  0.237E+03 14.94   2 15.00  8.19
  0.209E+00 -0.100E+00  0.192E+03 12.97   2 15.00  7.79
  0.214E+00 -0.100E+00  0.166E+03 11.57   2 15.00  7.39
  0.219E+00 -0.100E+00  0.161E+03 11.12   2 15.00  6.99
  0.224E+00 -0.100E+00  0.145E+03  8.90   2 15.00  6.59
  0.230E+00 -0.100E+00  0.127E+03  8.19   2 15.00  6.18
  0.271E+00 -0.100E+00  0.456E+02  8.66   2 15.00  2.99
  0.276E+00 -0.100E+00  0.289E+02 10.52   2 15.00  2.58
  0.281E+00 -0.100E+00  0.309E+02 10.36   2 15.00  2.18
  0.291E+00 -0.100E+00  0.199E+02  6.78   2 15.00  1.38
  0.312E+00 -0.100E+00  0.125E+02  6.62   2 15.00 -0.22
  0.343E+00 -0.100E+00  0.580E+01  8.10   2 15.00 -2.62
  0.384E+00 -0.100E+00  0.179E+01 15.20   2 15.00 -5.82
  0.436E+00 -0.100E+00  0.474E+00 37.97   2 15.00 -9.83
  0.183E+00  0.000E+00  0.424E+03 18.18   2 15.00  9.79
  0.188E+00  0.000E+00  0.350E+03 16.49   2 15.00  9.39
  0.194E+00  0.000E+00  0.363E+03 15.34   2 15.00  8.98
  0.199E+00  0.000E+00  0.248E+03 13.71   2 15.00  8.59
  0.204E+00  0.000E+00  0.208E+03 12.93   2 15.00  8.19
  0.209E+00  0.000E+00  0.212E+03 11.04   2 15.00  7.79
  0.214E+00  0.000E+00  0.148E+03  8.99   2 15.00  7.39
  0.219E+00  0.000E+00  0.144E+03  8.26   2 15.00  6.99
  0.224E+00  0.000E+00  0.143E+03  7.76   2 15.00  6.59
  0.230E+00  0.000E+00  0.114E+03  6.75   2 15.00  6.18
  0.271E+00  0.000E+00  0.397E+02  7.68   2 15.00  2.99
  0.276E+00  0.000E+00  0.331E+02  8.46   2 15.00  2.58
  0.281E+00  0.000E+00  0.274E+02  8.83   2 15.00  2.18
  0.291E+00  0.000E+00  0.216E+02  6.02   2 15.00  1.38
  0.312E+00  0.000E+00  0.151E+02  5.98   2 15.00 -0.22
  0.343E+00  0.000E+00  0.605E+01  6.15   2 15.00 -2.62
  0.384E+00  0.000E+00  0.186E+01 10.43   2 15.00 -5.82
  0.436E+00  0.000E+00  0.404E+00 25.00   2 15.00 -9.83
  0.183E+00  0.100E+00  0.431E+03 17.47   2 15.00  9.79
  0.188E+00  0.100E+00  0.347E+03 15.13   2 15.00  9.39
  0.194E+00  0.100E+00  0.386E+03 15.16   2 15.00  8.98
  0.199E+00  0.100E+00  0.274E+03 13.36   2 15.00  8.59
  0.204E+00  0.100E+00  0.294E+03 13.40   2 15.00  8.19
  0.209E+00  0.100E+00  0.223E+03  8.70   2 15.00  7.79
  0.214E+00  0.100E+00  0.169E+03  7.51   2 15.00  7.39
  0.219E+00  0.100E+00  0.137E+03  7.23   2 15.00  6.99
  0.224E+00  0.100E+00  0.137E+03  6.77   2 15.00  6.59
  0.230E+00  0.100E+00  0.126E+03  6.34   2 15.00  6.18
  0.271E+00  0.100E+00  0.460E+02  7.07   2 15.00  2.99
  0.276E+00  0.100E+00  0.370E+02  7.92   2 15.00  2.58
  0.281E+00  0.100E+00  0.302E+02  8.54   2 15.00  2.18
  0.291E+00  0.100E+00  0.231E+02  6.02   2 15.00  1.38
  0.312E+00  0.100E+00  0.147E+02  6.01   2 15.00 -0.22
  0.343E+00  0.100E+00  0.700E+01  6.00   2 15.00 -2.62
  0.384E+00  0.100E+00  0.224E+01  7.86   2 15.00 -5.82
  0.436E+00  0.100E+00  0.495E+00 17.23   2 15.00 -9.83
  0.183E+00  0.200E+00  0.560E+03 19.64   2 15.00  9.79
  0.188E+00  0.200E+00  0.405E+03 15.90   2 15.00  9.39
  0.194E+00  0.200E+00  0.315E+03 15.81   2 15.00  8.98
  0.199E+00  0.200E+00  0.274E+03 14.38   2 15.00  8.59
  0.204E+00  0.200E+00  0.318E+03 15.00   2 15.00  8.19
  0.209E+00  0.200E+00  0.214E+03  7.80   2 15.00  7.79
  0.214E+00  0.200E+00  0.162E+03  6.79   2 15.00  7.39
  0.219E+00  0.200E+00  0.159E+03  6.73   2 15.00  6.99
  0.224E+00  0.200E+00  0.135E+03  6.77   2 15.00  6.59
  0.230E+00  0.200E+00  0.133E+03  6.34   2 15.00  6.18
  0.271E+00  0.200E+00  0.571E+02  6.99   2 15.00  2.99
  0.276E+00  0.200E+00  0.411E+02  8.32   2 15.00  2.58
  0.281E+00  0.200E+00  0.345E+02  8.58   2 15.00  2.18
  0.291E+00  0.200E+00  0.251E+02  6.02   2 15.00  1.38
  0.312E+00  0.200E+00  0.164E+02  5.98   2 15.00 -0.22
  0.343E+00  0.200E+00  0.643E+01  6.00   2 15.00 -2.62
  0.384E+00  0.200E+00  0.220E+01  8.09   2 15.00 -5.82
  0.436E+00  0.200E+00  0.560E+00 15.68   2 15.00 -9.83
  0.183E+00  0.300E+00  0.419E+03 23.58   2 15.00  9.79
  0.188E+00  0.300E+00  0.396E+03 22.65   2 15.00  9.39
  0.194E+00  0.300E+00  0.331E+03 21.21   2 15.00  8.98
  0.199E+00  0.300E+00  0.377E+03 21.03   2 15.00  8.59
  0.204E+00  0.300E+00  0.401E+03 21.15   2 15.00  8.19
  0.209E+00  0.300E+00  0.193E+03  8.86   2 15.00  7.79
  0.214E+00  0.300E+00  0.153E+03  8.30   2 15.00  7.39
  0.219E+00  0.300E+00  0.151E+03  8.34   2 15.00  6.99
  0.224E+00  0.300E+00  0.134E+03  7.76   2 15.00  6.59
  0.230E+00  0.300E+00  0.149E+03  7.79   2 15.00  6.18
  0.271E+00  0.300E+00  0.595E+02  8.92   2 15.00  2.99
  0.276E+00  0.300E+00  0.403E+02 10.79   2 15.00  2.58
  0.281E+00  0.300E+00  0.313E+02 10.99   2 15.00  2.18
  0.291E+00  0.300E+00  0.232E+02  6.90   2 15.00  1.38
  0.312E+00  0.300E+00  0.159E+02  6.02   2 15.00 -0.22
  0.343E+00  0.300E+00  0.630E+01  7.13   2 15.00 -2.62
  0.384E+00  0.300E+00  0.238E+01  9.37   2 15.00 -5.82
  0.436E+00  0.300E+00  0.607E+00 18.12   2 15.00 -9.83
  0.214E+00  0.400E+00  0.198E+03 16.82   2 15.00  7.39
  0.219E+00  0.400E+00  0.173E+03 15.49   2 15.00  6.99
  0.224E+00  0.400E+00  0.149E+03 17.18   2 15.00  6.59
  0.230E+00  0.400E+00  0.986E+02 15.01   2 15.00  6.18
  0.271E+00  0.400E+00  0.711E+02 15.89   2 15.01  2.99
  0.276E+00  0.400E+00  0.287E+02 23.03   2 15.00  2.58
  0.281E+00  0.400E+00  0.368E+02 21.96   2 15.00  2.18
  0.291E+00  0.400E+00  0.247E+02 12.27   2 15.00  1.38
  0.312E+00  0.400E+00  0.146E+02 10.62   2 15.00 -0.22
  0.343E+00  0.400E+00  0.614E+01 11.55   2 15.00 -2.62
  0.384E+00  0.400E+00  0.195E+01 17.54   2 15.00 -5.82
  0.436E+00  0.400E+00  0.423E+00 33.57   2 15.00 -9.83


==> nutev <==
Parton distribution functions and benchmark cross sections at NNLO
S. Alekhin, J. Bluemlein and S. Moch

This file contains the data and systematic uncertainties (see Sec. 3 for details and use in PDF fit)
for the experiment
...
NUTEV:  PR D64, 112006 (2001)

The data on the reduced DIS dimuon production cross sections 

sig=[(1-y-(xyM_N)^2/Q2) F_2 + y^2/2 F_T +- y(1-y/2) xF_3] B_mu

and the correction for unmeasured phase space \eta (not applied to the data)

The correlated systematic errors come from 8 sources. All uncertainties are given in percent.

      x         Q2         y          sig     unc   \eta   NSE systematic uncertainty

neutrino beam

  0.210E-01  0.113E+01  0.324E+00  0.449E-01 17.61  0.368   8  3.01  1.34  3.48  3.54  2.45  3.59  7.87  2.74
  0.570E-01  0.306E+01  0.324E+00  0.529E-01 17.35  0.374   8  2.59  0.55  1.49  4.20  2.38  1.34  4.02  1.15
  0.101E+00  0.543E+01  0.324E+00  0.415E-01 16.20  0.383   8  5.74  1.18  1.42  2.85  1.66  2.00  4.53  0.24
  0.167E+00  0.897E+01  0.324E+00  0.325E-01 15.55  0.380   8  1.63  0.65  0.15  1.08  0.58  1.45  5.42  0.40
  0.326E+00  0.175E+02  0.324E+00  0.144E-01 14.17  0.393   8  4.44  1.46  1.18  2.36  2.85  1.60  2.92  0.07
  0.210E-01  0.194E+01  0.558E+00  0.786E-01 14.10  0.590   8  2.14  3.03  1.55  3.13  2.86  1.32  5.96  0.97
  0.570E-01  0.527E+01  0.558E+00  0.798E-01 13.16  0.590   8  1.74  0.83  1.74  2.43  2.19  2.84  5.59  0.24
  0.101E+00  0.934E+01  0.558E+00  0.783E-01 13.11  0.588   8  3.81  1.89  2.45  2.17  0.42  1.47  1.99  1.17
  0.167E+00  0.154E+02  0.558E+00  0.505E-01 12.71  0.596   8  1.80  1.50  3.40  1.60  0.71  1.29  3.32  0.36
  0.326E+00  0.302E+02  0.558E+00  0.228E-01 13.10  0.607   8  2.63  1.14  1.53  2.89  0.26  2.54  1.88  0.00
  0.210E-01  0.268E+01  0.771E+00  0.769E-01 14.71  0.693   8  5.71  1.01  1.68  1.57  1.90  5.64  1.63  0.17
  0.570E-01  0.729E+01  0.771E+00  0.911E-01 14.10  0.696   8  2.61  0.81  1.20  0.40  0.83  1.87  0.68  0.27
  0.101E+00  0.129E+02  0.771E+00  0.864E-01 14.35  0.695   8  2.56  0.08  1.04  1.45  1.55  2.23  1.87  0.35
  0.167E+00  0.213E+02  0.771E+00  0.694E-01 15.08  0.695   8  1.77  0.85  2.19  1.11  1.82  2.00  1.77  0.50
  0.326E+00  0.417E+02  0.771E+00  0.217E-01 16.90  0.706   8  0.78  0.55  1.89  1.29  1.15  2.26  2.30  0.32
  0.210E-01  0.223E+01  0.324E+00  0.116E+00 14.81  0.638   8  2.47  2.14  2.08  1.23  3.97  3.01  1.54  0.10
  0.570E-01  0.604E+01  0.324E+00  0.861E-01 14.21  0.639   8  4.69  1.30  2.72  1.48  3.83  2.44  3.29  0.39
  0.101E+00  0.107E+02  0.324E+00  0.854E-01 14.82  0.637   8  2.40  0.06  0.91  0.70  1.19  1.96  1.12  0.87
  0.167E+00  0.177E+02  0.324E+00  0.566E-01 14.11  0.648   8  3.84  0.90  2.65  2.07  1.41  1.03  1.98  1.26
  0.326E+00  0.346E+02  0.324E+00  0.255E-01 13.20  0.654   8  3.22  0.55  1.45  1.10  0.86  1.61  3.97  1.93
  0.210E-01  0.384E+01  0.558E+00  0.143E+00 15.13  0.777   8  1.79  0.93  1.48  0.52  3.58  2.67  3.99  0.73
  0.570E-01  0.104E+02  0.558E+00  0.135E+00 15.18  0.777   8  2.39  1.56  2.41  1.30  0.93  3.28  2.12  0.03
  0.101E+00  0.184E+02  0.558E+00  0.120E+00 15.88  0.779   8  2.65  0.60  0.26  0.69  0.49  2.00  1.66  0.82
  0.167E+00  0.305E+02  0.558E+00  0.762E-01 15.60  0.781   8  1.29  0.55  2.47  2.15  1.18  1.32  2.95  0.64
  0.326E+00  0.595E+02  0.558E+00  0.281E-01 15.17  0.786   8  3.62  0.53  3.91  2.52  2.66  2.42  1.31  0.78
  0.210E-01  0.530E+01  0.771E+00  0.152E+00 13.44  0.838   8  2.77  0.41  0.68  0.53  2.41  1.93  2.12  0.30
  0.570E-01  0.144E+02  0.771E+00  0.124E+00 13.15  0.832   8  1.94  2.55  2.14  1.65  1.55  1.35  2.87  0.14
  0.101E+00  0.255E+02  0.771E+00  0.107E+00 13.89  0.836   8  2.85  0.43  0.41  0.39  0.44  1.25  4.80  0.07
  0.167E+00  0.421E+02  0.771E+00  0.842E-01 15.46  0.845   8  1.24  0.58  0.84  0.75  0.39  2.23  3.83  0.86
  0.326E+00  0.823E+02  0.771E+00  0.308E-01 17.20  0.842   8  3.77  0.58  0.91  1.04  0.55  2.40  0.65  0.10
  0.210E-01  0.316E+01  0.324E+00  0.138E+00 14.37  0.730   8  2.46  0.70  1.30  1.17  1.51  4.38  2.76  0.30
  0.570E-01  0.857E+01  0.324E+00  0.143E+00 14.99  0.737   8  0.48  0.29  1.76  0.68  0.90  1.78  1.39  0.41
  0.101E+00  0.152E+02  0.324E+00  0.103E+00 14.50  0.738   8  2.16  0.58  1.33  0.54  0.81  2.87  1.13  0.09
  0.167E+00  0.251E+02  0.324E+00  0.762E-01 14.07  0.745   8  2.42  0.16  1.37  0.76  0.30  2.24  4.63  1.60
  0.326E+00  0.490E+02  0.324E+00  0.283E-01 12.18  0.751   8  6.07  1.27  3.28  0.95  1.80  2.89  3.60  1.06
  0.210E-01  0.544E+01  0.558E+00  0.166E+00 15.96  0.839   8  2.90  0.73  1.25  0.63  1.74  2.26  1.87  0.02
  0.570E-01  0.148E+02  0.558E+00  0.156E+00 16.36  0.841   8  3.81  0.06  1.45  1.91  1.03  3.40  1.95  1.16
  0.101E+00  0.261E+02  0.558E+00  0.113E+00 16.23  0.846   8  2.57  0.74  1.16  1.17  1.49  2.52  1.46  0.53
  0.167E+00  0.432E+02  0.558E+00  0.727E-01 15.81  0.846   8  4.81  0.95  0.95  1.07  0.99  2.17  2.85  0.18
  0.326E+00  0.844E+02  0.558E+00  0.315E-01 14.93  0.850   8  5.34  0.22  1.53  1.08  1.27  3.72  5.21  0.60
  0.210E-01  0.751E+01  0.771E+00  0.168E+00 13.28  0.885   8  7.54  0.61  2.27  3.04  0.86  3.31  3.87  0.63
  0.570E-01  0.204E+02  0.771E+00  0.140E+00 13.43  0.890   8  3.79  0.44  3.09  1.36  0.97  3.21  1.14  0.24
  0.101E+00  0.361E+02  0.771E+00  0.111E+00 13.84  0.888   8  1.42  0.27  1.66  1.27  1.90  2.27  1.73  0.14
  0.167E+00  0.597E+02  0.771E+00  0.896E-01 15.18  0.889   8  6.83  0.17  1.42  1.81  1.73  2.31  3.42  0.19
  0.326E+00  0.117E+03  0.771E+00  0.305E-01 16.63  0.891   8  9.07  0.20  1.15  1.60  2.00  3.47  4.91  0.10 

anti-neutrino beam

  0.420E-01  0.214E+01  0.349E+00  0.369E-01 27.98  0.353   8  2.06  4.47  3.15  2.58  2.03  3.39  5.04  2.14
  0.720E-01  0.367E+01  0.349E+00  0.337E-01 27.29  0.362   8  2.91  1.22  2.35  1.87  3.92  4.75  1.96  3.27
  0.114E+00  0.582E+01  0.349E+00  0.267E-01 26.48  0.362   8  0.86  1.35  1.20  0.49  2.66  3.79  1.99  0.71
  0.207E+00  0.106E+02  0.349E+00  0.797E-02 23.21  0.366   8  2.13 10.54  5.02  2.13  4.27  3.51  7.40  1.00
  0.150E-01  0.127E+01  0.579E+00  0.444E-01 21.74  0.564   8  0.81  2.48  2.12  0.29  0.56  3.31  1.89  0.65
  0.420E-01  0.356E+01  0.579E+00  0.504E-01 21.48  0.565   8  2.52  3.71  1.19  0.79  1.19  4.53  5.90  0.64
  0.720E-01  0.610E+01  0.579E+00  0.556E-01 21.60  0.569   8  0.97  3.63  1.12  1.08  3.02  2.05  5.11  1.03
  0.114E+00  0.965E+01  0.579E+00  0.295E-01 19.69  0.564   8  2.20  3.15  0.85  2.24  0.78  2.31  2.61  1.42
  0.207E+00  0.175E+02  0.579E+00  0.153E-01 20.58  0.575   8  1.44  3.34  1.31  1.70  1.44  2.95  7.14  1.05
  0.150E-01  0.170E+01  0.776E+00  0.539E-01 26.41  0.663   8  7.15 11.17  9.04  5.96 13.05  3.73  9.74  0.65
  0.420E-01  0.477E+01  0.776E+00  0.484E-01 23.47  0.652   8  1.55  5.81  8.14  1.22  6.76  4.32  9.75  1.03
  0.720E-01  0.817E+01  0.776E+00  0.454E-01 22.76  0.666   8  2.89  4.14  0.62  1.96  2.75  5.62  2.23  0.77
  0.114E+00  0.129E+02  0.776E+00  0.404E-01 23.93  0.665   8  3.34  3.47  0.87  1.34  1.83  4.90  5.23  0.64
  0.207E+00  0.235E+02  0.776E+00  0.143E-01 25.02  0.665   8  1.33  4.48  2.59  0.98  4.41  5.96  4.63  0.63
  0.150E-01  0.141E+01  0.349E+00  0.767E-01 23.82  0.593   8  0.78  3.21  2.10  0.95  1.15  4.68  7.30  2.09
  0.420E-01  0.396E+01  0.349E+00  0.739E-01 24.39  0.604   8  2.95  2.64  4.71  2.69  3.79  8.23  7.31  0.81
  0.720E-01  0.678E+01  0.349E+00  0.728E-01 24.65  0.602   8  0.87  2.25  1.61  1.19  4.98  1.57  2.65  1.54
  0.114E+00  0.107E+02  0.349E+00  0.427E-01 23.55  0.602   8  1.40  2.46  0.61  1.12  3.70  3.42  1.66  0.73
  0.207E+00  0.195E+02  0.349E+00  0.158E-01 22.02  0.611   8  7.07  7.13  6.94  3.97  3.72  3.91  0.95  0.88
  0.150E-01  0.234E+01  0.579E+00  0.118E+00 26.03  0.743   8  1.09  0.63  2.03  0.57  1.11  2.09  1.76  1.79
  0.420E-01  0.656E+01  0.579E+00  0.923E-01 24.64  0.747   8  0.56  3.18  1.85  1.35  2.38  2.94  3.08  1.03
  0.720E-01  0.112E+02  0.579E+00  0.723E-01 24.38  0.735   8  5.15  9.78  3.25  6.02  6.89  3.51  7.21  2.02
  0.114E+00  0.178E+02  0.579E+00  0.626E-01 25.40  0.745   8  3.27  4.23  0.69  4.41  7.53  4.88  1.72  1.32
  0.207E+00  0.323E+02  0.579E+00  0.223E-01 25.22  0.749   8  2.92  3.86  4.04  2.06  2.29  3.73  4.35  0.90
  0.150E-01  0.314E+01  0.776E+00  0.777E-01 21.57  0.801   8  0.71  2.19  2.11  0.46  1.92  4.89  2.73  1.96
  0.420E-01  0.879E+01  0.776E+00  0.108E+00 22.18  0.810   8  1.49  2.94  6.13  4.24  2.09  4.52  0.96  1.45
  0.720E-01  0.151E+02  0.776E+00  0.716E-01 22.35  0.811   8  1.22  1.69  5.39  1.03  1.44  4.33  8.02  0.63
  0.114E+00  0.239E+02  0.776E+00  0.527E-01 22.91  0.808   8  0.84  2.33  0.78  0.13  0.95  2.70  3.00  0.65
  0.207E+00  0.433E+02  0.776E+00  0.229E-01 26.42  0.809   8  1.44  4.94  2.71  0.52  3.46  4.77  2.10  0.83
  0.150E-01  0.223E+01  0.349E+00  0.102E+00 22.79  0.728   8  0.68  8.17  4.42  0.73  7.04  4.97  6.27  0.97
  0.420E-01  0.624E+01  0.349E+00  0.104E+00 22.91  0.732   8  5.69  4.88  1.83  2.23  3.11  2.03 10.19  1.77
  0.720E-01  0.107E+02  0.349E+00  0.713E-01 22.02  0.730   8  2.23  7.44  6.41  6.13  5.35  7.19  5.25  2.41
  0.114E+00  0.169E+02  0.349E+00  0.452E-01 22.09  0.732   8  0.31  5.51  1.77  0.66  0.71  6.15  3.49  0.75
  0.207E+00  0.308E+02  0.349E+00  0.278E-01 22.29  0.743   8  2.99  5.26  3.13  2.59  1.98  2.09  7.42  0.86
  0.150E-01  0.370E+01  0.579E+00  0.123E+00 26.21  0.840   8  7.09 16.66 13.36 11.16 12.55  8.51 14.70  0.69
  0.420E-01  0.104E+02  0.579E+00  0.104E+00 25.69  0.836   8  2.40  3.81  2.06  1.55  4.11  5.51  2.58  0.66
  0.720E-01  0.178E+02  0.579E+00  0.829E-01 26.04  0.835   8  4.23  3.63  2.86  4.27  3.32  5.27  5.83  1.47
  0.114E+00  0.281E+02  0.579E+00  0.562E-01 25.39  0.828   8  9.10 10.29 13.32  7.71 10.63  6.45  3.63  1.53
  0.207E+00  0.510E+02  0.579E+00  0.276E-01 26.94  0.841   8  2.32  4.63  2.35  2.50  2.57  4.45 12.02  0.80
  0.150E-01  0.496E+01  0.776E+00  0.912E-01 20.54  0.883   8  1.10  4.52  3.12  0.64  2.21  4.96  1.44  0.78
  0.420E-01  0.139E+02  0.776E+00  0.121E+00 21.66  0.876   8  1.18  3.63  2.21  0.79  2.60  5.26  3.88  1.05
  0.720E-01  0.238E+02  0.776E+00  0.101E+00 22.68  0.877   8  1.07  0.32  0.34  0.21  0.86  2.62  3.02  1.16
  0.114E+00  0.377E+02  0.776E+00  0.479E-01 22.26  0.877   8  2.34  4.03  4.17  1.77  4.26  5.88  1.75  0.83
  0.207E+00  0.684E+02  0.776E+00  0.184E-01 24.85  0.879   8  1.41  6.29  2.28  1.90  1.36  9.12  5.10  1.14

